Improved Spanning on Theta-5

We show an upper bound of $\frac{ \sin\left(\frac{3\pi}{10}\right) }{ \sin\left(\frac{2\pi}{5}\right)-\sin\left(\frac{3\pi}{10}\right) } <5.70$ on the spanning ratio of $\Theta_5$-graphs, improving on the previous best known upper bound of $9.96$ [Bose, Morin, van Renssen, and Verdonschot. The Theta-5-graph is a spanner. Computational Geometry, 2015.]

==> text/details/pentagon.tex <==
\section{Proof of Claim~\ref{claim:pentagon}}\label{claim:pentagon-details}

\input{text/theorem/pentagon}
\input{text/proof/pentagon}


==> text/details/proving-a-spanning-ratio-of-5.70.tex <==
%\section{Proving a spanning ratio of \texorpdfstring{$5.70$}{5.70} (missing proofs)}\label{down2K-details}

\section{Proof of Lemma~\ref{mainlemma1}}\label{mainlemma1-details}

In this section we show that $|ac|+|bd|+K|cd|-K|ab|\leq |ac'|+|bd'|+K|c'd'|-K|ab|$. See Figure~\ref{cdprime1}. Let $e$ be the intersection of $ac$ and $bd$, and let $e'$ be the intersection of $br'$ and $a\ell$. Observe that $\angle \ell e' r' =2\pi/5$, and thus we can see that $\angle dec\geq 2\pi/5$. This implies that $\angle dec$ cannot be the smallest angle in $\triangle dec$, since that would require $\angle dec\leq \pi/3$. Thus at least one of $\angle dce$ and $\angle edc$ is the smallest angle in $\triangle dec$. Since we have applied Transformation \ref{transformt5}, and can thus assume that $\alpha = \pi/10$, the cases are symmetric. We can therefore, without loss of generality, assume that $\angle dce$ is the smallest angle in $\triangle dec$.
\begin{figure}
	\begin{subfigure}[b]{0.5\textwidth}
		\centering
		\includegraphics[page =25]{figures/generalcase.pdf}
		\caption{Proof that $|c'd|\geq |cd|$.}%
		\label{cdprime1}
	\end{subfigure}%
	\begin{subfigure}[b]{0.5\textwidth}
		\centering
		\includegraphics[page =31]{figures/generalcase.pdf}
		\caption{Maximum of $\angle ed'c'$.}%
		\label{cdprime2}
	\end{subfigure}
	\begin{comment}	\qquad
	\begin{subfigure}[b]{0.45\textwidth}
	\centering
	\includegraphics[page =27]{figures/generalcase.pdf}
	\caption{Maximum of $\angle ed'c'$.}%
	\label{cdprime2}
	\end{subfigure}\end{comment}
	\caption{Finding the longest distance from $a$ to $b$ when $c$ and $d$ are in $P_{ab}$,}
\end{figure}

\restate{\LemmaMainOne*}

\begin{proof}
	Since $c$ lies on $ac'$ and $d$ lies on $bd'$, we have $|ac|\leq |ac'|$ and $|bd|\leq |bd'|$, and it is sufficient to show that $|cd|\leq |c'd'|$. We first show that $|cd|\leq |c'd|$. Since $\angle dce$ is the smallest angle in $\triangle dec$, $\angle dce< \pi/3$. That implies that $\angle c'cd >\pi/2$, which implies that $c'd$ is the longest side of triangle $\triangle cc'd$, and thus $|cd|\leq |c'd|$. See Fig.\ref{cdprime1}.

	We now show that $|c'd'|\geq |c'd|$. If $\angle c'dd' \geq \pi/2$, then $c'd'$ is the longest side of $\triangle c'dd'$, and $|c'd'|\geq |c'd|$ and we are done. Otherwise assume $\angle c'dd'< \pi/2$.

	The law of sines tells us that $\frac{|c'd'|}{\sin \angle c'dd'} =
	\frac{|c'd|}{\sin \angle dd'c'}$. Since $\sin \theta$ is an increasing
	function for $0\leq \theta <\pi/2$, showing that $\angle c'dd' \geq \angle
	dd'c'$ is sufficient to show $|c'd'|\geq |c'd|$, as it would imply both
	angles are $<\pi/2$. Observe that $\angle c'dd'\geq \angle c'ed'$ and
	$\angle ed'c'=\angle dd'c'$, thus it is sufficient to prove that $\angle
	c'ed'\geq \angle ed'c'$.

	Observe that $\angle ced =\angle c'ed' \geq 2\pi/5$. We now find the
	maximum of $\angle dd'c' = \angle ed'c'\leq 2\pi/5$. Observe that if $c'$
	moves left, $\angle ed'c'$ increases, thus assume $c'$ is at $p_1$. Let
	$O(bp_3c')$ be the circle through $b$, $p_3$, and $c'$ with center $o$.
	Observe that $o$ lies on $br'$. Observe that $\angle r'bd' = \pi/10$, thus
	$\angle r'op_3 = \pi/5$. Segment $or'$ makes an angle of $\pi/10$ with the
	horizontal line through $o$. Thus $od'$ makes an angle of $3\pi/10$ with
	the horizontal line through $o$, and thus the line tangent to $O(bp_3c')$
	at $p_3$ is the line supporting $\ell'r'$, since $\ell'r'$ makes an angle
	of $3\pi/10$ with the vertical line through $\ell'$. See
	Figure~\ref{cdprime2}. That implies that $[p_2,p_3)$ lies outside of
	$O(bp_3c')$, which means for every point $d'$, $\angle ed'c' \leq \angle
	ep_3c' = 2\pi/5$, and thus $\angle c'dd' \geq \angle dd'c'$ as required.\qed
\end{proof}




\begin{comment}


\begin{proof}	[Proof of Lemma \ref{mainlemma1}.]

We first claim that $\Phi \leq |ac|+|bd'|+K|cd'|-K|ab|$. Since $\angle edc$ is the smallest angle in $\triangle dec$, it must be that $\angle edc\leq \pi/3$. That implies that $\angle cdd' >\pi/2$, which implies that $|cd'|>|cd|$. Since $|bd'|\geq|bd|$, $\Phi =|ac|+|bd|+K|cd|-K|ab| \leq |ac|+|bd'|+K|cd'|-K|ab|$.

We now show that $|ac|+|bd'|+K|cd'|-K|ab|\leq |ac'|+|bd'|+K|c'd'|-K|ab|$. Since
$|ac|\leq|ac'|$ it is enough to show that $|c'd'|\geq|cd'|$. If $\angle
c'cd'\geq \pi/2$, then $|c'd'|$ is the largest edge in $\triangle cc'd'$, and
$|c'd'|\geq|cd'|$. Thus assume $\angle c'cd'< \pi/2$. We have $\angle c'cd'
\geq \angle c'ed' \geq 2\pi/5$. We claim that $\angle ed'c' \geq \pi/10$, and
since $\angle c'ed' \geq 2\pi/5$, it must be that $\angle d'c'e \leq \pi/2$.
Since $\sin\beta$ is increasing in $\beta$, $0\leq\beta\leq \pi/2$, the law of
sines implies that $K|c'd'|\geq |K|cd'|$ if $\sin\angle d'c'e \leq \sin\angle
c'cd'$. Since $\angle c'ed'\leq \angle c'cd'$, it is sufficient to show that
$\angle d'c'e \leq \angle c'ed'$. See Figure~\ref{worstcase3}. We can increase
$\angle d'c'e$ by moving $d'$ to $p_2$. If we place $c'$ at $p_0$, observe that
the circle through $a$, $c'$ and $d'$ is tangent to $\ell r$ at $c'$. Thus as
$c'$ moves left with $a$ and $d'$ fixed, $\angle d'c'e$ decreases, so it is
maximized when $d'$ is at $p_2$ and $c'$ is at $p_0$, at which point $\angle
d'c'e = 2\pi/5$. Since $\angle c'ed' \geq 2\pi/5$, $\angle d'c'e \leq \angle
c'ed'$ as required.

We are left with showing $\angle ed'c' \geq \pi/10$.	For a fixed $d'$, $\angle ed'c'$ is decreased as $c'$ moves right. Thus assume $c'$ is at $p_0$. Observe that when $d'$ is at $p_3$, the circle through $b$, $d'$ and $c'$ intersects $\ell'r'$ at $d'$ and $a$, thus any point $d''\neq d'$ on $p_2p_3$ is outside of the circle, which implies $\angle ed'c'$ is decreasing as $d'$ moves towards $p_2$. Thus $\angle ed'c'$ is minimized when $d'=p_2$ and $c'=p_0$, at which point $\angle ed'c'=\pi/10$. See Figure~\ref{edcangle}.

\end{proof}

\begin{figure}
\begin{subfigure}[b]{0.5\textwidth}
\centering
\includegraphics[page = 5]{figures/generic1.pdf}
\caption{The worst case angles for $\triangle ec'd'$.}%
\label{worstcase3}
\end{subfigure}%
\begin{subfigure}[b]{0.5\textwidth}
\centering
\includegraphics[page = 19]{figures/generalcase.pdf}
\caption{Minimum value of $\angle ed'c'$.}%
\label{edcangle}
\end{subfigure}
\caption{}
\end{figure}
\end{comment}


\section{Proof of Lemma~\ref{mainlemma2}}\label{mainlemma2-details}

Observe that $|ap_1|+K|p_1p_3|+|p_3b| = |ap_0|+K|p_0p_2|+|p_2b|$ when $\alpha =
\pi/10$, since $T_{ab}$ and $T_{ba}$ are the same size and the cases are
symmetric.
%
We prove that
\begin{align*}
	\Phi' = |ac'|+K|c'd'|+|d'b|-K|ab| &\leq |ap_1|+K|p_1p_3|+|p_3b| -K|ab| = \Phi'' \\
							  &= |ap_0|+K|p_0p_2|+|p_2b|-K|ab|.
\end{align*}


\begin{figure}
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[page = 23]{figures/generalcase.pdf}
		\caption{The point $q$ such that $|p_1q|=|c'd'|$ lies between $d'$ and $p_2$.}%
		\label{worstcase2}
	\end{subfigure}%
	\hfill
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[page = 24]{figures/generalcase.pdf}
		\caption{We look at the change in $|d'p_3|+K|c'd'|$ with respect to $\theta$.}%
		\label{final}
	\end{subfigure}
	\caption{}
\end{figure}

\restate{\LemmaMainTwo*}

\begin{proof}

	(Figure~\ref{worstcase})
	%
	Without loss of generality, we assume that $|p_1c'|\leq|p_2d'|$. We
	show that $\Phi'$ is maximized when $c'=p_1$ and $d'=p_3$.

	(Figure~\ref{worstcase2})
	%
	Observe that $|p_1p_2|\leq |c'd'|\leq |p_1p_3|$.
	Let $z$ be a point on $p_2p_3$ that moves from $p_2$ to $p_3$, and observe
	that $|p_1z|$ takes on every value from $|p_1p_2|$ to $|p_2p_3|$. Thus
	there must be a point $q$ on $p_2p_3$ such that $|p_1q|=|c'd'|$.

	We claim that $|ap_1|+|bq| \geq |ac'|+|bd'|$, which
	implies that $\Phi' \leq |ap_1| + K|p_1q| + |qb| - K|ab|$.

	Observe $|ap_1|\geq |ac'|$, since $\angle p_1c'a >\pi/2$, making $ap_1$ the
	longest edge in triangle $\triangle ac'p_1$. We claim that $q$ is between
	$d'$ and $p_2$, and thus $|bq|\geq |bd'|$ since $\angle bd'q > \pi/2$.
	By contradiction, assume that $q$ is between $d'$ and
	$p_3$. Since $|p_1c'|\leq|p_2d'|$, $\angle qd'c' >\pi/2$, which implies
	that $|c'q|>|c'd'|$. Also note that $\angle qd'p_1 >\pi/2$, which implies
	$|p_1q|>|c'q|>|c'd'|$, a contradiction. Thus assuming that $c'=p_1$ and
	$d'=q$ does not decrease $\Phi'$.

	Now, given that $c'$ is on $p_1$, we show that $\Phi' \leq
	|ac'|+|bp_3|+K|c'p_3|$, that is, when $d'$ is on $p_3$. To do this we
	define another function $\Phi^* = |ac'|+|d'p_3|+|p_3b|+K|c'd'|-K|ab|$. See
	Figure~\ref{final}. Since $|bd'|\leq |d'p_3|+|p_3b|$ by the triangle
	inequality, $\Phi' \leq \Phi^*$, and observe that $\Phi'
	=\Phi^*=\Phi''$ when $d'=p_3$. We show that $\Phi^*$ is maximized
	when $d'=p_3$, thus implying that $\Phi'$ is also maximized when $d'=p_3$,
	and $\Phi'\leq \Phi''$. Let $\theta = \angle p_2p_1d'$. We allow $d'$ to
	move along $p_2p_3$ until $d'$ is on $p_3$, and fix all other points, and
	observe how $\Phi^*$ changes with $\theta$.

	We first rewrite $\Phi^*$ as $\Phi^*=
	|ac'|+|p_2p_3|-|p_2d'|+|p_3b|+K|c'd'|-K|ab|$. Using the sine law we get
	$|p_2d'|=\frac{\sin\theta}{\sin(2\pi/5-\theta)}|p_1p_2|$, and $|c'd'| =
	\frac{\sin(3\pi/5)}{\sin(2\pi/5-\theta)}|p_1p_2|$. All other terms of
	$\Phi^*$ have fixed values with respect to $\theta$. Thus

	\begin{align}
	\frac{d\Phi^*}{d\theta}
	&= \frac{d}{d\theta}\left( K\frac{\sin(3\pi/5)}{\sin(2\pi/5-\theta)}|p_1p_2| -\frac{\sin\theta}{\sin(2\pi/5-\theta)}|p_1p_2|\right)\nonumber\\
	&= \frac{K\cos(2\pi/5-\theta)\sin(3\pi/5)-\cos\theta\sin(2\pi/5-\theta) - \sin\theta\cos(2\pi/5-\theta)}{\sin^2(2\pi/5-\theta)}|p_1p_2|\nonumber\\
	&= \frac{K\cos(2\pi/5-\theta)\sin(3\pi/5)-\sin(2\pi/5)}{\sin^2(2\pi/5-\theta)}|p_1p_2|.\label{number}
	\end{align}

	Observe that $0\leq \theta \leq 3\pi/10$. The denominator of \eqref{number}
	is always positive. The numerator of \eqref{number} is minimized at $\theta
	= 0$, which for $K\geq5.70$ is positive. Thus \eqref{number} is always
	positive for $0\leq \theta\leq 3\pi/10$, thus $\Phi^*$ is increasing in
	$\theta$, and is maximized when $d'=p_3$, as required.
	%
	Thus $\Phi' \leq \Phi^* \leq \Phi'' = |ap_1|+K|p_1p_3|+|p_3b|-K|ab|$ as required.\qed
\end{proof}


==> text/details/transformation.tex <==

\section{Proof of Lemma~\ref{posofc}}\label{sec:details:transformation}
\input{text/theorem/transformation}
\begin{wrapfigure}[\ifarxiv 2 \else 15\fi]{r}{0.20\textwidth}
	\centering
	\includegraphics[page=1]{figures/transformation.pdf}
	\caption{The values used in the proof of Lemma~\ref{posofc}.}%
	\label{ctransform-lemma-details}
\end{wrapfigure}
\noindent
\begin{minipage}[t]{0.75\textwidth}
\input{text/proof/transformation}
\end{minipage}


==> text/main.tex <==
\input{text/introduction}
\input{text/preliminaries}
\input{text/analysis}
\input{text/proving-a-spanning-ratio-of-5.70}
\input{text/conclusion}

